A Conceptual Model for the Analysis of Investigation Elements in Games

This paper presents the 4E conceptual model, developed to formally analyze investigation games from a game design perspective. The model encompasses four components: Exploration, Elicitation, Experimentation, and Evaluation. Grounded Theory was employed as the methodology for constructing the model, allowing for an in-depth understanding of the underlying concepts. The resulting model was then compared to existing literature, and its contributions were thoroughly discussed. Overall, the 4E model presents a comprehensive framework for understanding investigation games elements. It's application in two real-world scenarios demonstrates its practical relevance.

==> tables/tab_clue_analysis.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{p{2cm}p{4cm}p{4cm}}
    \hline
        Subcategoria & Anotações do Jogo & Anotações do Avaliador \\ \hline
        Clue Discrimination & A clue is easy to spot as soon as you discover if a card is in the table. & "Ao ver que uma carta está presente na mesa, é objetivo e nítido que aquilo representa uma pista. Agora se está mais próximo de criar melhores experimentos." \\ 
        Clue Storage & """Marking off your CLUE sheet""" & A forma do jogador registrar a pista.\\ 
        Eval. Feedback & """The player on your left must be the first to try to answer your question. If they have any of the cards you asked about they must show one of them to you secretly.""" & "Depois de um experimento normal (CLUE question), existe um mecanismo de validação parcial de UMA das partes da sua pergunta (arma, pessoa ou local)." \\ 
        Eval. Feedback & """After the accusation without letting anyone else see check the cards in the Envelope [for validation]""" & Depois de uma acusação você sabe se acertou ou errou. \\ 
        Exper. Guidance & """To win you must be the first player to find out which suspect weapon and room cards are in the Murder Envelope.""" & "O mistério principal do jogo é muito bem definido, que já direciona o jogador." \\ 
        Exper. Guidance & """A CLUE question is about one suspect, one weapon and the room you’ve just entered.""" & "A experimentação do jogo segue um formato específico de afirmar uma arma, um local e uma pessoa."  \\ 
        Exper. Scheduling & """If you entered a room  you must stop and ask a CLUE question""" Toda entrada em uma sala dispara o momento de experimentar uma hipótese. \\ 
        Exper. Scheduling & """Accusation can be done at any time""" & "Acusação é um tipo de experimento de alto risco: se errar, o jogador sai do jogo. Ela pode ocorrer a qualquer momento, mesmo que por chute. Ela é um tipo de " \\ 
        Explor. Space & """Roll the dice and move your character token that number of spaces around the board.""" & "Os personagens andam pela mansão, visitando os lugares para tentar descobrir pistas do assassinato." \\ 
        Explor. Progress & Each player can (in it's turn) move freely to any room and explore in any order &"Não existe ordem fixa para a exploração, inclusive cada jogador tem sua ""própria"" jornada." \\ \hline
    \end{tabular}
    \caption{a}
    \label{a}
\end{table}
